Non-normal Recurrent Neural Network (nnRNN): learning long time dependencies while improving expressivity with transient dynamics

A recent strategy to circumvent the exploding and vanishing gradient problem in RNNs, and to allow the stable propagation of signals over long time scales, is to constrain recurrent connectivity matrices to be orthogonal or unitary. This ensures eigenvalues with unit norm and thus stable dynamics and training. However this comes at the cost of reduced expressivity due to the limited variety of orthogonal transformations. We propose a novel connectivity structure based on the Schur decomposition and a splitting of the Schur form into normal and non-normal parts. This allows to parametrize matrices with unit-norm eigenspectra without orthogonality constraints on eigenbases. The resulting architecture ensures access to a larger space of spectrally constrained matrices, of which orthogonal matrices are a subset. This crucial difference retains the stability advantages and training speed of orthogonal RNNs while enhancing expressivity, especially on tasks that require computations over ongoing input sequences.

==> OLD_PTB_table.tex <==
\begin{table}[h!]
\begin{center}
\small
\begin{tabular}{c|cc|cc|cc|cc}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{Test BPC / Accuracy} \\
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{Fixed \# params ($\sim$1.32M)} & \multicolumn{2}{c|}{Fixed \# hidden units  ($N=1024$)} \\
Model                 & $T_{PTB}=150$                     & $T_{PTB}=300$            & $T_{PTB}=150$          & $T_{PTB}=300$           \\ \hline
RNN                   & 2.89 $\pm$ 0.002 / 40.01 $\pm$ 0.026                   &  2.90 $\pm$ 0.0016 / 39.97 $\pm$ 0.02 5          &2.89 $\pm$ 0.002 / 40.01 $\pm$ 0.026                   &  2.90 $\pm$ 0.0016 / 39.97 $\pm$ 0.025  \\
RNN-orth                   & 1.62 $\pm$ 0.0039/66.29 $\pm$ 0.07                   & 1.66 $\pm$ 0.0055 / 65.53 $\pm$ 0.09           & 1.62 $\pm$ 0.0039/66.29 $\pm$ 0.07                   & 1.66 $\pm$ 0.0055 / 65.53 $\pm$ 0.09       \\
EURNN                 &  1.61 $\pm$ 0.0005 / 65.68 $\pm$ 0.0017      & 1.62 $\pm$ 0.0014 /65.55 $\pm$ 0.0020         & 1.69 $\pm$ 0.0007 / 64.01 $\pm$ 0.0022        &  1.68 $\pm$ 0.0009 /64.20 $\pm$ 0.0028         \\
ExpRNN                & 1.49 $\pm$ 0.008 / 68.07 $\pm$ 0.15          & 1.52 $\pm$ 0.0014 / 67.58 $\pm$ 0.04           & 1.51 $\pm$ 0.005 / 67.51 $\pm$ 0.11     & 1.55 $\pm$ 0.0008 / 66.89 $\pm$ 0.024/        \\
nnRNN                 &{\bf 1.47 $\pm$ 0.0036 / 68.78 $\pm$ 0.0006}  & {\bf 1.49 $\pm$ 0.0020 / 68.52 $\pm$ 0.0004} & {\bf 1.47 $\pm$ 0.0036 / 68.78 $\pm$ 0.0006}  & {\bf 1.49 $\pm$ 0.0020 / 68.52 $\pm$ 0.0004}    \\\hline
% LSTM                  & 1.39 / 69.84          & 1.38 / 70.45     & 1.37 / 70.60                & 1.42 / 69.95               
\end{tabular}
\end{center}
\label{ptb_table}
\caption{PTB test performance: Bit per Character (BPC) and Test Accuracy, for sequence lengths $T_{PTB}=150, 300$. Two comparisons across models shown: fixed number of parameters (left), and fixed number of hidden units (right).Error range indicates standard error of the mean. \\ }
\end{table}

==> PTB150_table.tex <==
\begin{table}[h!]
\begin{center}
\small
\begin{tabular}{c|ll}%|cc|cc}
\multicolumn{1}{l}{} & \multicolumn{2}{c}{Test BPC / Accuracy ($T_{PTB}=150$)} \\
% \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{Fixed \# params ($\sim$1.32M)} & \multicolumn{2}{c|}{Fixed \# hidden units  ($N=1024$)} \\
Model                 & Fixed \# params ($\sim$1.32M)                                & Fixed \# hidden units  ($N=1024$)    \\ \hline
RNN                   & 2.89 $\pm$ 0.002 / 40.01 $\pm$ 0.026                             &2.89 $\pm$ 0.002 / 40.01 $\pm$ 0.026                     \\
RNN-orth                   & 1.62 $\pm$ 0.004 / 66.29 $\pm$ 0.07                              & 1.62 $\pm$ 0.004 / 66.29 $\pm$ 0.07                          \\
EURNN                 &  1.61 $\pm$ 0.001 / 65.68 $\pm$ 0.002               & 1.69 $\pm$ 0.001 / 64.01 $\pm$ 0.002                 \\
expRNN                & 1.49 $\pm$ 0.008 / 68.07 $\pm$ 0.15                     & 1.51 $\pm$ 0.005 / 67.51 $\pm$ 0.11             \\
nnRNN                 &{\bf 1.47 $\pm$ 0.003 / 68.78 $\pm$ 0.0006}   & {\bf 1.47 $\pm$ 0.003 / 68.78 $\pm$ 0.0006}      \\\hline
% LSTM                  & 1.39 / 69.84          & 1.38 / 70.45     & 1.37 / 70.60                & 1.42 / 69.95               
\end{tabular}
\end{center}
\label{ptb150_table}
\caption{PTB test performance: Bit per Character (BPC) and Test Accuracy, for sequence lengths $T_{PTB}=150$. Two comparisons across models shown: fixed number of parameters (left), and fixed number of hidden units (right). Error range indicates standard error of the mean. \\ }
\end{table}

==> PTB300_table.tex <==
\begin{table}[h!]
\begin{center}
\small
\begin{tabular}{c|ll}%|cc|cc}
\multicolumn{1}{l}{} & \multicolumn{2}{c}{Test BPC / Accuracy} \\
Model                 & Fixed \# params ($\sim$1.32M)                                & Fixed \# hidden units  ($N=1024$)    \\ \hline
RNN                   &  2.90 $\pm$ 0.0016 / 39.97 $\pm$ 0.02 5                      &  2.90 $\pm$ 0.0016 / 39.97 $\pm$ 0.025  \\
RNN-orth                    & 1.66 $\pm$ 0.0055 / 65.53 $\pm$ 0.09                & 1.66 $\pm$ 0.0055 / 65.53 $\pm$ 0.09       \\
EURNN        & 1.62 $\pm$ 0.0014 / 65.55 $\pm$ 0.0020         &  1.68 $\pm$ 0.0009 / 64.20 $\pm$ 0.0028         \\
expRNN             & 1.52 $\pm$ 0.0014 / 67.58 $\pm$ 0.04          & 1.55 $\pm$ 0.0008 / 66.89 $\pm$ 0.024/        \\
nnRNN        & {\bf 1.49 $\pm$ 0.0020 / 68.52 $\pm$ 0.0004} & {\bf 1.49 $\pm$ 0.0020 / 68.52 $\pm$ 0.0004}    \\\hline
% LSTM                  & 1.39 / 69.84          & 1.38 / 70.45     & 1.37 / 70.60                & 1.42 / 69.95               
\end{tabular}
\end{center}
\label{ptb_table}
\caption{PTB test performance: Bit per Character (BPC) and Test Accuracy, for sequence lengths $T_{PTB}=300$. Two comparisons across models shown: fixed number of parameters (left), and fixed number of hidden units (right). Error range indicates standard error of the mean. \\ }
\end{table}

==> PTB_table.tex <==
\begin{table}[h!]
\begin{center}
\small
\begin{tabular}{c|cc|cc|cc|cc}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{Test BPC / Accuracy} \\
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{Fixed \# params ($\sim$1.32M)} & \multicolumn{2}{c|}{Fixed \# hidden units  ($N=1024$)} \\
Model                 & $T_{PTB}=150$                     & $T_{PTB}=300$            & $T_{PTB}=150$          & $T_{PTB}=300$           \\ \hline
RNN                   & 2.89 $\pm$ 0.002 / 40.01 $\pm$ 0.026                   &  2.90 $\pm$ 0.0016 / 39.97 $\pm$ 0.025          &2.89 $\pm$ 0.002 / 40.01 $\pm$ 0.026                   &  2.90 $\pm$ 0.002 / 39.97 $\pm$ 0.025  \\
RNN-orth                   & 1.62 $\pm$ 0.004/66.29 $\pm$ 0.07                   & 1.66 $\pm$ 0.006 / 65.53 $\pm$ 0.09           & 1.62 $\pm$ 0.004/66.29 $\pm$ 0.07                   & 1.66 $\pm$ 0.006 / 65.53 $\pm$ 0.09       \\
EURNN                 &  1.61 $\pm$ 0.001 / 65.68 $\pm$ 0.002      & 1.62 $\pm$ 0.001 /65.55 $\pm$ 0.002         & 1.69 $\pm$ 0.001 / 64.01 $\pm$ 0.002        &  1.68 $\pm$ 0.001 /64.20 $\pm$ 0.003         \\
expRNN                & 1.49 $\pm$ 0.008 / 68.07 $\pm$ 0.15          & 1.52 $\pm$ 0.001 / 67.58 $\pm$ 0.04           & 1.51 $\pm$ 0.005 / 67.51 $\pm$ 0.11     & 1.55 $\pm$ 0.001 / 66.89 $\pm$ 0.024/        \\
nnRNN                 &{\bf 1.47 $\pm$ 0.003 / 68.78 $\pm$ 0.0006}  & {\bf 1.49 $\pm$ 0.002 / 68.52 $\pm$ 0.0004} & {\bf 1.47 $\pm$ 0.003 / 68.78 $\pm$ 0.0006}  & {\bf 1.49 $\pm$ 0.002 / 68.52 $\pm$ 0.0004}    \\\hline
% LSTM                  & 1.39 / 69.84          & 1.38 / 70.45     & 1.37 / 70.60                & 1.42 / 69.95               
\end{tabular}
\end{center}
\label{ptb_table}
\caption{PTB test performance: Bit per Character (BPC) and Test Accuracy, for sequence lengths $T_{PTB}=150, 300$. Two comparisons across models shown: fixed number of parameters (left), and fixed number of hidden units (right). Error range indicates standard error of the mean. \\ }
\end{table}

==> PTBacc_RebuttalTable.tex <==
\begin{table}[h!]
\begin{center}
\small
\begin{tabular}{c|ll|ll}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{Test Accuracy} \\
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{Fixed \# params ($\sim$1.32M)} & \multicolumn{2}{c}{Fixed \# hidden units  ($N=1024$)} \\
Model                 & $T_{PTB}=150$                     & $T_{PTB}=300$            & $T_{PTB}=150$          & $T_{PTB}=300$           \\ \hline
RNN                   &40.01 $\pm$ 0.026                   & 39.97 $\pm$ 0.025          &40.01 $\pm$ 0.026            &39.97 $\pm$ 0.025  \\
RNN-orth                   &66.29 $\pm$ 0.07                   &65.53 $\pm$ 0.09           &66.29 $\pm$ 0.07            &65.53 $\pm$ 0.09   \\
EURNN                 &65.68 $\pm$ 0.002      &65.55 $\pm$ 0.002         &64.01 $\pm$ 0.002        &64.20 $\pm$ 0.003         \\
expRNN                &68.07 $\pm$ 0.15          &67.58 $\pm$ 0.04           &67.51 $\pm$ 0.11     &66.89 $\pm$ 0.024        \\
nnRNN                 &{\bf68.78 $\pm$ 0.0006}  & {\bf68.52 $\pm$ 0.0004} & {\bf68.78 $\pm$ 0.0006}  & {\bf68.52 $\pm$ 0.0004}    \\
nnRNN-$\gamma =1$  &    68.93 $\pm$ 0.0007*      & 68.21**  &    68.93 $\pm$ 0.0007*      & 68.21**    \\
nnRNN-$\gamma =0.958$  &   68.81 $\pm$ 0.0008   &  68.42 $\pm$ 0.0013  &   68.81 $\pm$ 0.0008   &  68.42 $\pm$ 0.0013 \\ \hline 
% LSTM                  & 1.39 / 69.84          & 1.38 / 70.45     & 1.37 / 70.60                & 1.42 / 69.95               
\end{tabular}
\end{center}
\label{ptb_acc_table}
\caption{PTB test performance: Test Accuracy, for sequence lengths $T_{PTB}=150, 300$. Two comparisons across models shown: fixed number of parameters (left), and fixed number of hidden units (right). Error range indicates standard error of the mean. *: Indicates 3 of 5 runs experienced instability, **: Indictaes 4 of 5 runs experienced instability \\ }
\end{table}

==> PTBbpc_Rebuttal_Table.tex <==
\begin{table}[h!]
\vspace*{-1.5mm}
\begin{center}
\small
\begin{tabular}{c|ll|ll}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{Test Bit per Character (BPC)} \\
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{Fixed \# params ($\sim$1.32M)} & \multicolumn{2}{c}{Fixed \# hidden units  ($N=1024$)} \\
Model                 & $T_{PTB}=150$                     & $T_{PTB}=300$            & $T_{PTB}=150$          & $T_{PTB}=300$           \\ \hline
RNN                   & 2.89 $\pm$ 0.002                    &  2.90 $\pm$ 0.0016          &2.89 $\pm$ 0.002                    &  2.90 $\pm$ 0.002   \\
RNN-orth                   & 1.62 $\pm$ 0.004                 & 1.66 $\pm$ 0.006         & 1.62 $\pm$ 0.004                  & 1.66 $\pm$ 0.006       \\
EURNN                 &  1.61 $\pm$ 0.001      & 1.62 $\pm$ 0.001          & 1.69 $\pm$ 0.001        &  1.68 $\pm$ 0.001         \\
expRNN                & 1.49 $\pm$ 0.008          & 1.52 $\pm$ 0.001           & 1.51 $\pm$ 0.005      & 1.55 $\pm$ 0.001       \\
nnRNN                 &{\bf 1.47 $\pm$ 0.003 }  & {\bf 1.49 $\pm$ 0.002} & {\bf 1.47 $\pm$ 0.003}  & {\bf 1.49 $\pm$ 0.002 }    \\
nnRNN-$\gamma =1$  &    1.46 $\pm$ 0.005*      & 1.49** &    1.46 $\pm$ 0.005*      & 1.49**   \\
nnRNN-$\gamma =0.958$  &   1.47 $\pm$ 0.005   &  1.49 $\pm$ 0.008 &   1.47 $\pm$ 0.005   &  1.49 $\pm$ 0.008 \\ \hline 
% LSTM                  & 1.39 / 69.84          & 1.38 / 70.45     & 1.37 / 70.60                & 1.42 / 69.95               
\end{tabular}
\end{center}
\label{ptb_table}
\caption{PTB test performance: Bit per Character (BPC), for sequence lengths $T_{PTB}=150, 300$. Two comparisons across models shown: fixed number of parameters (left), and fixed number of hidden units (right). Error range indicates standard error of the mean.}
\vspace*{-2mm}
\end{table}

==> PTBbpc_newRebut.tex <==
\begin{table}[h!]
\vspace*{-1.5mm}
% \begin{center}
% \small
% \begin{tabular}{c|ll|ll}
\begin{tabular}[t]{c|ll|ll}%{p{2cm}>{\bfseries}p{2.5cm}p{3cm}}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{Test Bit per Character (BPC)} \\
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{Fixed \# params ($\sim$1.32M)} & \multicolumn{2}{c}{Fixed \# hidden units  ($N=1024$)} \\
Model                 & $T_{PTB}=150$                     & $T_{PTB}=300$            & $T_{PTB}=150$          & $T_{PTB}=300$           \\ \hline
% RNN                   & 2.89 $\pm$ 0.002                    &  2.90 $\pm$ 0.0016          &2.89 $\pm$ 0.002                    &  2.90 $\pm$ 0.002   \\
% RNN-orth                   & 1.62 $\pm$ 0.004                 & 1.66 $\pm$ 0.006         & 1.62 $\pm$ 0.004                  & 1.66 $\pm$ 0.006       \\
% EURNN                 &  1.61 $\pm$ 0.001      & 1.62 $\pm$ 0.001          & 1.69 $\pm$ 0.001        &  1.68 $\pm$ 0.001         \\
% expRNN                & 1.49 $\pm$ 0.008          & 1.52 $\pm$ 0.001           & 1.51 $\pm$ 0.005      & 1.55 $\pm$ 0.001       \\
% nnRNN                 &{\bf 1.47 $\pm$ 0.003 }  & {\bf 1.49 $\pm$ 0.002} & {\bf 1.47 $\pm$ 0.003}  & {\bf 1.49 $\pm$ 0.002 }    \\
nnRNN-$\gamma =1$  &    1.46 $\pm$ 0.005*      & 1.49** &    1.46 $\pm$ 0.005*      & 1.49**   \\
nnRNN-$\gamma =0.958$  &   1.47 $\pm$ 0.005   &  1.49 $\pm$ 0.008 &   1.47 $\pm$ 0.005   &  1.49 $\pm$ 0.008 \\ \hline 
% LSTM                  & 1.39 / 69.84          & 1.38 / 70.45     & 1.37 / 70.60                & 1.42 / 69.95               
\end{tabular}
% \end{center}
\label{ptb_table}
% \caption{PTB test performance: Bit per Character (BPC), for sequence lengths $T_{PTB}=150, 300$. Two comparisons across models shown: fixed number of parameters (left), and fixed number of hidden units (right). Error range indicates standard error of the mean.}
\vspace*{-2mm}
\end{table}
